Accelerating COVID-19 research with graph mining and transformer-based learning

In 2020, the White House released the, "Call to Action to the Tech Community on New Machine Readable COVID-19 Dataset," wherein artificial intelligence experts are asked to collect data and develop text mining techniques that can help the science community answer high-priority scientific questions related to COVID-19. The Allen Institute for AI and collaborators announced the availability of a rapidly growing open dataset of publications, the COVID-19 Open Research Dataset (CORD-19). As the pace of research accelerates, biomedical scientists struggle to stay current. To expedite their investigations, scientists leverage hypothesis generation systems, which can automatically inspect published papers to discover novel implicit connections. We present an automated general purpose hypothesis generation systems AGATHA-C and AGATHA-GP for COVID-19 research. The systems are based on graph-mining and the transformer model. The systems are massively validated using retrospective information rediscovery and proactive analysis involving human-in-the-loop expert analysis. Both systems achieve high-quality predictions across domains (in some domains up to 0.97% ROC AUC) in fast computational time and are released to the broad scientific community to accelerate biomedical research. In addition, by performing the domain expert curated study, we show that the systems are able to discover on-going research findings such as the relationship between COVID-19 and oxytocin hormone.

==> preface.tex <==
% This section allows us to modify preloaded package properties
\makeatletter
% These magic runes make comment's appear inline
% These also need to be above the other magic runes
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\usepackage{regexpatch}
\xpatchcmd{\@todo}{\setkeys{todonotes}{#1}}{\setkeys{todonotes}{inline,#1}}{}{}

% These magic runes make the new changes package work with comments
\usepackage{comment}
\let\wfs@comment@comment\comment
\let\comment\@undefined
\usepackage{changes}
\let\wfs@changes@comment\comment
\let\comment\@undefined
\newcommand\comment{%
    \ifthenelse{\equal{\@currenvir}{comment}}
    {\wfs@comment@comment}
    {\wfs@changes@comment}%
}
\makeatother

% Typical preloader time

\usepackage{amsmath}
\usepackage{hyperref}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{outlines}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{float}
\usepackage{nicefrac}
\usepackage{url}
\usepackage{booktabs}
\usepackage{listings}
\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
  frame=single,
  breaklines=true,
  tabsize=2,
  breakautoindent=true,
}

% Changes Authors
\definechangesauthor[name="Ankit Kulshrestha", color=blue]{ak}
\definechangesauthor[name="Ilya Tyagin", color=cyan]{it}
\definechangesauthor[name="Justin Sybrandt", color=green]{js}
\definechangesauthor[name="Ilya Safro", color=red]{is}


\newcommand{\pymoliererepo}{
\href{http://sybrandt.com/2020/agatha}
{sybrandt.com/2020/agatha}
}
\newcommand{\pymoliere}{AGATHA}

% These are shortcuts for leaving specific changes comments
\newcommand{\note}[2]{\added[id=#1, comment={#2}]{}}

% Ankit's add, delete, replace
\newcommand{\Aak}[1]{\added[id=ak]{#1}}
\newcommand{\Dak}[1]{\deleted[id=ak]{#1}}
\newcommand{\Rak}[2]{\replaced[id=ak]{#1}{#2}}

% Justin's add, delete, replace
\newcommand{\Ajs}[1]{\added[id=js]{#1}}
\newcommand{\Djs}[1]{\deleted[id=js]{#1}}
\newcommand{\Rjs}[2]{\replaced[id=js]{#1}{#2}}

% ITyagin's add, delete replace
\newcommand{\Ait}[1]{\added[id=it]{#1}}
\newcommand{\Dit}[1]{\deleted[id=it]{#1}}
\newcommand{\Rit}[2]{\replaced[id=it]{#1}{#2}}

% ISafro's add, delete, replace
\newcommand{\Ais}[1]{\added[id=is]{#1}}
\newcommand{\Dis}[1]{\deleted[id=is]{#1}}
\newcommand{\Ris}[2]{\replaced[id=is]{#1}{#2}}

% THIS ALLOWS FOR CONDITIONAL COMMENTS
%\newif\ifthesis
% Comment/ un-comment as needed
%\thesisfalse
%\thesistrue

\newif\ifthesis
\thesistrue % use false for AAAI, true for full thesis

% % Comment out a block of text for KDD (but keep for thesis) with this syntax:
% \ifthesis
% % <Text to comment out>
% \else
% % <Optional replacement for KDD Version>
% \fi

%\thesisfalse
%\thesistrue


\hyphenation{
    AG-A-THA
}

% These magic runes make everything denser

\setlength{\textfloatsep}{3pt}
\setlength{\floatsep}{3pt}
\setlength{\belowdisplayskip}{3pt} \setlength{\belowdisplayshortskip}{3pt}
\setlength{\abovedisplayskip}{3pt} \setlength{\abovedisplayshortskip}{3pt}

% \settopmatter{authorsperrow=4}

\newcommand{\sysnameo}{AGATHA-O }
\newcommand{\sysnamec}{AGATHA-C }
\newcommand{\sysnamegp}{AGATHA-GP }

==> tables/case_study_numbers.tex <==
\begin{table}[h]
    \centering
    \caption{\label{tab:case_study_numbers}Scores for valid recently published connections obtained by different \pymoliere{} models. Reported average values for 100 runs and standard deviation.}
    \setlength{\tabcolsep}{.3em}
    \begin{tabular}{lccc}
    
    \toprule
    {} &            \sysnameo &            \sysnamec &            \sysnamegp \\
    \midrule
    COVID-19:Melatonin &  0.63 ± 0.03 &  0.91 ± 0.03 &  0.78 ± 0.03 \\
    COVID-19:Oxytocin  &  0.75 ± 0.03 &  0.98 ± 0.02 &  0.81 ± 0.02 \\
    COVID-19:BST2 gene &  0.41 ± 0.01 &  0.88 ± 0.03 &  0.74 ± 0.03 \\
    \bottomrule
    \vspace*{1mm}
    \end{tabular}

\end{table}

==> tables/graph_metrics.tex <==
\begin{table}[!t]
    \centering
    \caption{Graph size information (M = millions, B = billions).}
    \begin{tabular}{l c c c}
    \toprule
         & \multicolumn{3}{c}{Counts} \\
    \cmidrule {2-4}
        %Node Type & \sysnameo & \sysnamec & \sysnamegp \\
        Node Type & O & C & GP \\
    \midrule
        %Sentence & \multicolumn{3}{c}{190,605}\\
        %Sentence & 190,605,378 & 190,605,405 & 190,605,409\\
        Sentence & 190.6 M. & 190.6 M.  & 190.6 M. \\
       
        %Predicate & 24,189,417 & 36,284,104 & 38,669,519\\
        Predicate & 24.2 M. & 36.3 M. & 38.7 M.\\
        
        %Lemma & 16,830,025 & 16,053,858 & 16,054,753\\
        Lemma & 16.8 M. & 16.1 M. & 16.1 M.\\
        
        %Entity & 41,681,372 & 43,231,254 & 43,237,799\\
        Entity & 41.7 M. & 43.2 M. & 43.2 M.\\
        
        %Coded Term & 538,588 & 855,351 & 855,351\\
        Coded Term & 538,588 & 855,351 & 855,351\\
        
        %$n$-Grams & 212,922 & 326,864 & 333,575\\
        $n$-Grams & 212.922 & 326.864 & 333.575\\
    \midrule
        %Total Nodes &  274,057,702 & 287,356,836 & 289,756,406\\
        Total Nodes &  274,1 M. & 287.4 M. & 289.8 M.\\
        %Total Edges &  13,517,219,828 & 13,500,291,256 & 13,538,669,794\\
        Total Edges &  13.52 B. & 13.5 B. & 13.53 B.\\
    %\midrule
        %Mean degree & 49.32 & 46.98 & 46.72 \\
        %Median degree & 40 & 39 & 38 \\
    \bottomrule
    \end{tabular}
    %\parbox[t]{\textwidth}{\footnotesize
      %\textit{Note:}
      %All numbers presented in thousands}
    \label{tab:graph_metrics}
\end{table}

==> tables/model_size.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{lr}
        \pymoliere-512 Parameters & 1,313,280 \\
        \pymoliere-512 Embeddings & 10,115,707,904 \\
        \pymoliere-256 Parameters & 328, 960 \\
        \pymoliere-256 Embeddings & 5,057,853,952 \\
         
    \end{tabular}
    \caption{Model Size. Because embeddings are trained separately from the hypothesis prediction model, both numbers are listed. Embedding numbers correspond to the amount of floating-point values associated with predicate and coded-term embeddings needed to use the model.}
    \label{tab:model_size}
\end{table}
